Noise-Robust Keyword Spotting through Self-supervised Pretraining

Voice assistants are now widely available, and to activate them a keyword spotting (KWS) algorithm is used. Modern KWS systems are mainly trained using supervised learning methods and require a large amount of labelled data to achieve a good performance. Leveraging unlabelled data through self-supervised learning (SSL) has been shown to increase the accuracy in clean conditions. This paper explores how SSL pretraining such as Data2Vec can be used to enhance the robustness of KWS models in noisy conditions, which is under-explored. Models of three different sizes are pretrained using different pretraining approaches and then fine-tuned for KWS. These models are then tested and compared to models trained using two baseline supervised learning methods, one being standard training using clean data and the other one being multi-style training (MTR). The results show that pretraining and fine-tuning on clean data is superior to supervised learning on clean data across all testing conditions, and superior to supervised MTR for testing conditions of SNR above 5 dB. This indicates that pretraining alone can increase the model's robustness. Finally, it is found that using noisy data for pretraining models, especially with the Data2Vec-denoising approach, significantly enhances the robustness of KWS models in noisy conditions.

==> incl/temp.tex <==
% \begin{table}[ht]
%     \centering
%     \footnotesize
%     \setlength\tabcolsep{1.5mm}
%     \begin{tabular}{@{}lllllllll@{}}
%     \toprule
%         SNR                                         & -10    & -5     & 0      & 5      & 10     & 15     & 20     & clean  \\ \midrule
%         \makecell[l]{ Baseline- \\ Clean }          & 0.121 & 0.214 & 0.347 & 0.495 & 0.621 & 0.708 & 0.761 & 0.833 \\ 
%         \makecell[l]{ Baseline- \\ MTR }            & 0.231 & 0.383 & 0.538 & 0.654 & 0.728 & 0.767 & 0.793 & 0.810 \\ 
%         \makecell[l]{ Data2Vec - \\ clean }         & 0.176 & 0.323 & 0.508 & 0.673 & 0.780 & 0.839 & 0.871 & \textbf{0.906} \\ 
%         \makecell[l]{ Data2Vec - \\ cln+noisy }     & 0.301 & 0.490 & 0.663 & 0.775 & 0.831 & 0.863 & 0.879 & 0.888 \\ 
%         \makecell[l]{ Data2Vec - \\ noisy }         & 0.291 & 0.475 & 0.647 & 0.759 & 0.819 & 0.850 & 0.877 & 0.874 \\
%         \makecell[l]{ Data2Vec - \\ denoising }     & \textbf{0.315} & \textbf{0.502} & \textbf{0.670} & \textbf{0.777} & \textbf{0.836} & \textbf{0.864} & \textbf{0.880} & 0.890 \\ \bottomrule
%     \end{tabular}
%     % \begin{tabular}{@{}lllllll@{}}
%     %     \multicolumn{6}{c}{\textbf{KWT-2}}\\
%     %     \toprule
%     %     % &  & & \multicolumn{3}{c}{Data2vec pretraining} \\ \cline{4-6}
%     %     SNR    & \makecell[l]{ Baseline- \\ Clean training } & \makecell[l]{ Baseline- \\ MST } & \makecell[l]{ Data2Vec - \\ clean } & \makecell[l]{ Data2Vec - \\ pre: clean } & \makecell[l]{ Data2Vec - \\ pre: noisy } & \makecell[l]{ Data2Vec - \\ denoising }\\ \midrule
%     %     -10   & 0.1209 & 0.2308 & 0.1760 & 0.3008 & 0.2908 & 0.3152 \\
%     %     -5    & 0.2141 & 0.3832 & 0.3225 & 0.4898 & 0.4749 & 0.5019 \\
%     %     0     & 0.3472 & 0.5376 & 0.5081 & 0.6625 & 0.6472 & 0.6701 \\
%     %     5     & 0.4953 & 0.6538 & 0.6725 & 0.7747 & 0.7589 & 0.7769 \\
%     %     10    & 0.6211 & 0.7281 & 0.7801 & 0.8309 & 0.8188 & 0.8362 \\
%     %     15    & 0.7077 & 0.7670 & 0.8389 & 0.8628 & 0.8498 & 0.8643 \\
%     %     20    & 0.7619 & 0.7931 & 0.8708 & 0.8793 & 0.8669 & 0.8800 \\
%     %     clean & 0.8330 & 0.8104 & 0.9061 & 0.8875 & 0.8742 & 0.8904 \\
        
%     %     \bottomrule
%     % \end{tabular}
%     \caption{Shows the accuracy of the six models trained using KWT-2, when tested on data with known noises. The first two rows are the baseline tests. The last four rows are pretrained in different ways using the Data2Vec framework.}
%     \label{tab:KWT-2_seen}
% \end{table}

% \begin{table}[ht]
%     \centering
%     \footnotesize
%     \setlength\tabcolsep{1.5mm}
%     \begin{tabular}{@{}lllllllll@{}}
%         \toprule
%         SNR                                         & -10    & -5     & 0      & 5      & 10     & 15     & 20     & clean  \\ \midrule
%         \makecell[l]{ Baseline- \\ Clean }          & 0.127 & 0.222 & 0.359 & 0.497 & 0.612 & 0.691 & 0.746 & 0.814 \\ 
%         \makecell[l]{ Baseline- \\ MTR }            & 0.214 & 0.351 & 0.502 & 0.615 & 0.690 & 0.734 & 0.761 & 0.779 \\ 
%         \makecell[l]{ Data2Vec - \\ clean }         & 0.146 & 0.262 & 0.421 & 0.582 & 0.702 & 0.774 & 0.817 & 0.863 \\ 
%         \makecell[l]{ Data2Vec - \\ cln+noisy }     & 0.266 & 0.436 & 0.594 & 0.710 & 0.774 & 0.813 & 0.831 & 0.838 \\ 
%         \makecell[l]{ Data2Vec - \\ noisy }         & 0.267 & 0.432 & 0.592 & 0.705 & 0.769 & 0.807 & 0.827 & 0.844 \\
%         \makecell[l]{ Data2Vec - \\ denoising }     & 0.276 & 0.451 & 0.613 & 0.726 & 0.796 & 0.829 & 0.853 & 0.861 \\ \bottomrule
%     \end{tabular}
%     % \begin{tabular}{@{}lllllll@{}}
%     %     \multicolumn{6}{c}{\textbf{KWT-3}}\\
%     %     \toprule
%     %     % &  & & \multicolumn{3}{c}{Data2vec pretraining} \\ \cline{4-6}
%     %     SNR    & \makecell[l]{ Baseline- \\ Clean training } & \makecell[l]{ Baseline- \\ MST } & \makecell[l]{ Data2Vec - \\ clean } & \makecell[l]{ Data2Vec - \\ pre: clean } & \makecell[l]{ Data2Vec - \\ pre: noisy } & \makecell[l]{ Data2Vec - \\ denoising }\\ \midrule
%     %     -10   & 0.1267 & 0.2135 & 0.1460 & 0.2659 & 0.2671 & 0.2755 \\
%     %     -5    & 0.2219 & 0.3509 & 0.2615 & 0.4356 & 0.4320 & 0.4509 \\
%     %     0     & 0.3589 & 0.5024 & 0.4207 & 0.5943 & 0.5922 & 0.6127 \\
%     %     5     & 0.4969 & 0.6149 & 0.5816 & 0.7096 & 0.7049 & 0.7263 \\
%     %     10    & 0.6121 & 0.6902 & 0.7022 & 0.7740 & 0.7692 & 0.7958 \\
%     %     15    & 0.6917 & 0.7335 & 0.7740 & 0.8129 & 0.8074 & 0.8291 \\
%     %     20    & 0.7455 & 0.7611 & 0.8166 & 0.8309 & 0.8272 & 0.8527 \\
%     %     clean & 0.8142 & 0.7789 & 0.8630 & 0.8375 & 0.8442 & 0.8613 \\
        
%     %     \bottomrule
%     % \end{tabular}
%     \caption{Accuracy of the six models trained using KWT-3, when tested on data with known noises. The first two rows are the baseline tests. The last four rows are pretrained in different ways using the Data2Vec framework.}
%     \label{tab:KWT-3_seen}
% \end{table}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/results/all_seen.png}
%     \caption{Summary of the results when testing the models, outlined in \Cref{tab:names_of_models}, on data with seen noises}
%     \label{fig:all_seen}
% \end{figure}

    % \begin{tabular}{@{}llllllll@{}}
    %     \multicolumn{6}{c}{\textbf{KWT-1}}\\
    %     \toprule
    %     % &  & & \multicolumn{3}{c}{Data2vec pretraining} \\ \cline{4-6}
    %     SNR    & \makecell[l]{ Baseline- \\ Clean training } & \makecell[l]{ Baseline- \\ MTR } & \makecell[l]{ Data2Vec - \\ clean } & \makecell[l]{ Data2Vec - \\ pre: clean } & \makecell[l]{ Data2Vec - \\ pre: noisy } & \makecell[l]{ Data2Vec - \\ denoising } \\ \midrule
    %     -10   & 0.1328 & 0.2363 & 0.1742 & 0.2981 & 0.2969 & 0.3100 \\
    %     -5    & 0.2360 & 0.3896 & 0.2965 & 0.4775 & 0.4771 & 0.5004 \\
    %     0     & 0.3702 & 0.5358 & 0.4625 & 0.6382 & 0.6375 & 0.6650 \\
    %     5     & 0.5094 & 0.6478 & 0.6240 & 0.7493 & 0.7495 & 0.7685 \\
    %     10    & 0.6285 & 0.7199 & 0.7428 & 0.8120 & 0.8075 & 0.8247 \\
    %     15    & 0.7166 & 0.7600 & 0.8084 & 0.8413 & 0.8386 & 0.8538 \\
    %     20    & 0.7691 & 0.7832 & 0.8483 & 0.8598 & 0.8574 & 0.8677 \\
    %     clean & 0.8321 & 0.7995 & 0.8865 & 0.8661 & 0.8719 & 0.8756 \\
        
    %     \bottomrule
    % \end{tabular}


    % \begin{tabular}{@{}lllllll@{}}
    %     \multicolumn{6}{c}{\textbf{KWT-3}}\\
    %     \toprule
    %     % &  & & \multicolumn{3}{c}{Data2vec pretraining} \\ \cline{4-6}
    %     SNR    & \makecell[l]{ Baseline- \\ Clean training } & \makecell[l]{ Baseline- \\ MST } & \makecell[l]{ Data2Vec - \\ clean } & \makecell[l]{ Data2Vec - \\ pre: clean } & \makecell[l]{ Data2Vec - \\ pre: noisy } & \makecell[l]{ Data2Vec - \\ denoising }\\ \midrule
    %     -10   & 0.09691 & 0.1618 & 0.1131 & 0.2055 & 0.1931 & 0.2137 \\
    %     -5    & 0.1915 & 0.3076 & 0.2234 & 0.3975 & 0.3875 & 0.4121 \\
    %     0     & 0.3399 & 0.4680 & 0.4119 & 0.5885 & 0.5881 & 0.6000 \\
    %     5     & 0.4985 & 0.5997 & 0.5953 & 0.7091 & 0.7081 & 0.7238 \\
    %     10    & 0.6199 & 0.6766 & 0.7184 & 0.7763 & 0.7737 & 0.7944 \\
    %     15    & 0.7036 & 0.7301 & 0.7852 & 0.8124 & 0.8099 & 0.8303 \\
    %     20    & 0.7493 & 0.7566 & 0.8219 & 0.8299 & 0.8293 & 0.8511 \\
    %     clean & 0.8142 & 0.7789 & 0.8630 & 0.8375 & 0.8442 & 0.8613 \\
        
    %     \bottomrule
    % \end{tabular}

% \begin{table}[ht]
%     \centering
%     \footnotesize
%     \setlength\tabcolsep{1.5mm}
%     \begin{tabular}{@{}lllllllll@{}}
%         \toprule
%         SNR                                         & -10    & -5     & 0      & 5      & 10     & 15     & 20     & clean  \\ \midrule
%         \makecell[l]{ Baseline- \\ Clean }          & 0.100 & 0.197 & 0.351 & 0.527 & 0.650 & 0.730 & 0.776 & 0.833 \\ 
%         \makecell[l]{ Baseline- \\ MTR }            & 0.169 & 0.345 & 0.520 & 0.643 & 0.721 & 0.765 & 0.791 & 0.810 \\ 
%         \makecell[l]{ Data2Vec - \\ clean }         & 0.117 & 0.270 & 0.498 & 0.684 & 0.792 & 0.852 & 0.879 & 0.906 \\ 
%         \makecell[l]{ Data2Vec - \\ cln+noisy }     & 0.225 & 0.448 & 0.651 & 0.771 & 0.832 & 0.863 & 0.881 & 0.888 \\ 
%         \makecell[l]{ Data2Vec - \\ noisy }         & 0.217 & 0.430 & 0.624 & 0.754 & 0.819 & 0.853 & 0.871 & 0.874 \\
%         \makecell[l]{ Data2Vec - \\ denoising }     & 0.235 & 0.460 & 0.660 & 0.775 & 0.833 & 0.867 & 0.882 & 0.890 \\ \bottomrule
%     \end{tabular}
%     % \begin{tabular}{@{}lllllll@{}}
%     %     \multicolumn{6}{c}{\textbf{KWT-2}}\\
%     %     \toprule
%     %     % &  & & \multicolumn{3}{c}{Data2vec pretraining} \\ \cline{4-6}
%     %     SNR    & \makecell[l]{ Baseline- \\ Clean training } & \makecell[l]{ Baseline- \\ MST } & \makecell[l]{ Data2Vec - \\ clean } & \makecell[l]{ Data2Vec - \\ pre: clean } & \makecell[l]{ Data2Vec - \\ pre: noisy } & \makecell[l]{ Data2Vec - \\ denoising }\\ \midrule
%     %     -10   & 0.09959 & 0.1686 & 0.1171 & 0.2254 & 0.2169 & 0.2351 \\
%     %     -5    & 0.1972 & 0.3447 & 0.2698 & 0.4483 & 0.4303 & 0.4603 \\
%     %     0     & 0.3506 & 0.5196 & 0.4978 & 0.6512 & 0.6242 & 0.6602 \\
%     %     5     & 0.5273 & 0.6434 & 0.6839 & 0.7712 & 0.7536 & 0.7749 \\
%     %     10    & 0.6504 & 0.7214 & 0.7920 & 0.8323 & 0.8193 & 0.8328 \\
%     %     15    & 0.7301 & 0.7653 & 0.8521 & 0.8629 & 0.8532 & 0.8672 \\
%     %     20    & 0.7759 & 0.7914 & 0.8790 & 0.8812 & 0.8707 & 0.8820 \\
%     %     clean & 0.8330 & 0.8104 & 0.9061 & 0.8875 & 0.8742 & 0.8904 \\
        
%     %     \bottomrule
%     % \end{tabular}
%     \caption{Shows the accuracy of the six models trained using KWT-2, when tested on data with unknown noises. The first two rows are the baseline tests. The last four rows are pretrained in different ways using the Data2Vec framework.}
%     \label{tab:KWT-2_unseen}
% \end{table}

% \begin{table}[ht] 
%     \centering
%     \footnotesize
%     \setlength\tabcolsep{1.5mm}
%     \begin{tabular}{@{}lllllllll@{}}
%         \toprule
%         SNR                                         & -10    & -5     & 0      & 5      & 10     & 15     & 20     & clean  \\ \midrule
%         \makecell[l]{ Baseline- \\ Clean }          & 0.097 & 0.192 & 0.340 & 0.499 & 0.620 & 0.704 & 0.749 & 0.814 \\ 
%         \makecell[l]{ Baseline- \\ MTR }            & 0.161 & 0.308 & 0.468 & 0.600 & 0.677 & 0.730 & 0.757 & 0.779 \\ 
%         \makecell[l]{ Data2Vec - \\ clean }         & 0.113 & 0.223 & 0.412 & 0.595 & 0.718 & 0.785 & 0.822 & 0.863 \\ 
%         \makecell[l]{ Data2Vec - \\ cln+noisy }     & 0.206 & 0.398 & 0.589 & 0.709 & 0.776 & 0.812 & 0.830 & 0.838 \\ 
%         \makecell[l]{ Data2Vec - \\ noisy }         & 0.193 & 0.388 & 0.588 & 0.708 & 0.774 & 0.801 & 0.829 & 0.844 \\
%         \makecell[l]{ Data2Vec - \\ denoising }     & 0.214 & 0.412 & 0.600 & 0.724 & 0.794 & 0.830 & 0.851 & 0.861 \\ \bottomrule
%     \end{tabular}
%     % \begin{tabular}{@{}lllllll@{}}
%     %     \multicolumn{6}{c}{\textbf{KWT-3}}\\
%     %     \toprule
%     %     % &  & & \multicolumn{3}{c}{Data2vec pretraining} \\ \cline{4-6}
%     %     SNR    & \makecell[l]{ Baseline- \\ Clean training } & \makecell[l]{ Baseline- \\ MST } & \makecell[l]{ Data2Vec - \\ clean } & \makecell[l]{ Data2Vec - \\ pre: clean } & \makecell[l]{ Data2Vec - \\ pre: noisy } & \makecell[l]{ Data2Vec - \\ denoising }\\ \midrule
%     %     -10   & 0.09691 & 0.1618 & 0.1131 & 0.2055 & 0.1931 & 0.2137 \\
%     %     -5    & 0.1915 & 0.3076 & 0.2234 & 0.3975 & 0.3875 & 0.4121 \\
%     %     0     & 0.3399 & 0.4680 & 0.4119 & 0.5885 & 0.5881 & 0.6000 \\
%     %     5     & 0.4985 & 0.5997 & 0.5953 & 0.7091 & 0.7081 & 0.7238 \\
%     %     10    & 0.6199 & 0.6766 & 0.7184 & 0.7763 & 0.7737 & 0.7944 \\
%     %     15    & 0.7036 & 0.7301 & 0.7852 & 0.8124 & 0.8099 & 0.8303 \\
%     %     20    & 0.7493 & 0.7566 & 0.8219 & 0.8299 & 0.8293 & 0.8511 \\
%     %     clean & 0.8142 & 0.7789 & 0.8630 & 0.8375 & 0.8442 & 0.8613 \\
        
%     %     \bottomrule
%     % \end{tabular}
%     \caption{Shows the accuracy of the six models trained using KWT-3, when tested on data with unknown noises. The first two rows are the baseline tests. The last four rows are pretrained in different ways using the Data2Vec framework.}
%     \label{tab:KWT-3_unseen}
% \end{table}

% % \begin{figure}[ht]
% %     \centering
% %     \includegraphics[width=0.45\textwidth]{figures/results/kwt1_known.png}
% %     \caption{KWT1}
% %     \label{fig:KWT-1_seen}
% % \end{figure}
% % \begin{figure}[ht]
% %     \centering
% %     \includegraphics[width=0.45\textwidth]{figures/results/kwt2_known.png}
% %     \caption{KWT2}
% %     \label{fig:KWT-2_seen}
% % \end{figure}

% % \begin{figure}[ht]
% %     \centering
% %     \includegraphics[width=0.45\textwidth]{figures/results/kwt3_known.png}
% %     \caption{KWT3}
% %     \label{fig:KWT-3_seen}
% % \end{figure}


% \begin{table}[ht] 
%     \centering
%     \footnotesize
%     \setlength\tabcolsep{1.5mm}
%     \begin{tabular}{@{}lllllll@{}}
%         \toprule
%          & \multicolumn{2}{c}{KWT-1} & \multicolumn{2}{c}{KWT-2} & \multicolumn{2}{c}{KWT-3} \\
%          & Seen & Unseen & Seen & Unseen & Seen & Unseen \\ 
%          \hline
%          Baseline-Clean & 0.524 & 0.532 & 0.513 & 0.521 & 0.509 & 0.502 \\
%          Baseline-MTR & 0.609 & 0.592 & 0.613 & 0.596 & 0.581 & 0.560 \\
%          Data2Vec-Clean & 0.606 & 0.501 & 0.635 & 0.625 & 0.571 & 0.566 \\
%          Data2Vec-Clean + Noisy & 0.693 & 0.676 & 0.711 & 0.695 & 0.658 & 0.645 \\ 
%          Data2Vec-Noisy & 0.692 & 0.676 & 0.699 & 0.680 & 0.655 & 0.641  \\
%          Data2Vec-Denoising & \textbf{0.708} & \textbf{0.688} & \textbf{0.717} & \textbf{0.700} & \textbf{0.676} & \textbf{0.661} \\ 
%         \bottomrule
%     \end{tabular}
%     % \begin{tabular}{@{}lllllll@{}}
%     %     \multicolumn{6}{c}{\textbf{KWT-3}}\\
%     %     \toprule
%     %     % &  & & \multicolumn{3}{c}{Data2vec pretraining} \\ \cline{4-6}
%     %     SNR    & \makecell[l]{ Baseline- \\ Clean training } & \makecell[l]{ Baseline- \\ MST } & \makecell[l]{ Data2Vec - \\ clean } & \makecell[l]{ Data2Vec - \\ pre: clean } & \makecell[l]{ Data2Vec - \\ pre: noisy } & \makecell[l]{ Data2Vec - \\ denoising }\\ \midrule
%     %     -10   & 0.09691 & 0.1618 & 0.1131 & 0.2055 & 0.1931 & 0.2137 \\
%     %     -5    & 0.1915 & 0.3076 & 0.2234 & 0.3975 & 0.3875 & 0.4121 \\
%     %     0     & 0.3399 & 0.4680 & 0.4119 & 0.5885 & 0.5881 & 0.6000 \\
%     %     5     & 0.4985 & 0.5997 & 0.5953 & 0.7091 & 0.7081 & 0.7238 \\
%     %     10    & 0.6199 & 0.6766 & 0.7184 & 0.7763 & 0.7737 & 0.7944 \\
%     %     15    & 0.7036 & 0.7301 & 0.7852 & 0.8124 & 0.8099 & 0.8303 \\
%     %     20    & 0.7493 & 0.7566 & 0.8219 & 0.8299 & 0.8293 & 0.8511 \\
%     %     clean & 0.8142 & 0.7789 & 0.8630 & 0.8375 & 0.8442 & 0.8613 \\
        
%     %     \bottomrule
%     % \end{tabular}
%     \caption{Mean accuracies of the models by averaging the accuracies at every noise level, including clean condition. The highest accuracies are highlighted with bold font.}
%     \label{tab:mean_scores}
% \end{table}

    % \begin{tabular}{@{}lllllll@{}}
    %     \multicolumn{6}{c}{\textbf{KWT-1}}\\
    %     \toprule
    %     % &  & & \multicolumn{3}{c}{Data2vec pretraining} \\ \cline{4-6}
    %     SNR    & \makecell[l]{ Baseline- \\ Clean training } & \makecell[l]{ Baseline- \\ MST } & \makecell[l]{ Data2Vec - \\ clean } & \makecell[l]{ Data2Vec - \\ pre: clean } & \makecell[l]{ Data2Vec - \\ pre: noisy } & \makecell[l]{ Data2Vec - \\ denoising }\\ \midrule
    %     -10   & 0.1039 & 0.1812 & 0.1299 & 0.2222 & 0.2247 & 0.2189 \\
    %     -5    & 0.2117 & 0.3411 & 0.2538 & 0.4315 & 0.4338 & 0.4459 \\
    %     0     & 0.3764 & 0.5170 & 0.4607 & 0.6287 & 0.6271 & 0.6483 \\
    %     5     & 0.5478 & 0.6397 & 0.6431 & 0.7478 & 0.7443 & 0.7654 \\
    %     10    & 0.6614 & 0.7136 & 0.7573 & 0.8079 & 0.8080 & 0.8229 \\
    %     15    & 0.7376 & 0.7614 & 0.8238 & 0.8438 & 0.8426 & 0.8554 \\
    %     20    & 0.7829 & 0.7841 & 0.8545 & 0.8613 & 0.8562 & 0.8712 \\
    %     clean & 0.8321 & 0.7995 & 0.8865 & 0.8661 & 0.8719 & 0.8756 \\
        
    %     \bottomrule
    % \end{tabular}    % \begin{tabular}{@{}lllllll@{}}
    %     \multicolumn{6}{c}{\textbf{KWT-1}}\\
    %     \toprule
    %     % &  & & \multicolumn{3}{c}{Data2vec pretraining} \\ \cline{4-6}
    %     SNR    & \makecell[l]{ Baseline- \\ Clean training } & \makecell[l]{ Baseline- \\ MST } & \makecell[l]{ Data2Vec - \\ clean } & \makecell[l]{ Data2Vec - \\ pre: clean } & \makecell[l]{ Data2Vec - \\ pre: noisy } & \makecell[l]{ Data2Vec - \\ denoising }\\ \midrule
    %     -10   & 0.1039 & 0.1812 & 0.1299 & 0.2222 & 0.2247 & 0.2189 \\
    %     -5    & 0.2117 & 0.3411 & 0.2538 & 0.4315 & 0.4338 & 0.4459 \\
    %     0     & 0.3764 & 0.5170 & 0.4607 & 0.6287 & 0.6271 & 0.6483 \\
    %     5     & 0.5478 & 0.6397 & 0.6431 & 0.7478 & 0.7443 & 0.7654 \\
    %     10    & 0.6614 & 0.7136 & 0.7573 & 0.8079 & 0.8080 & 0.8229 \\
    %     15    & 0.7376 & 0.7614 & 0.8238 & 0.8438 & 0.8426 & 0.8554 \\
    %     20    & 0.7829 & 0.7841 & 0.8545 & 0.8613 & 0.8562 & 0.8712 \\
    %     clean & 0.8321 & 0.7995 & 0.8865 & 0.8661 & 0.8719 & 0.8756 \\
        
    %     \bottomrule
    % \end{tabular}
